Provable Reinforcement Learning with a Short-Term Memory

Real-world sequential decision making problems commonly involve partial observability, which requires the agent to maintain a memory of history in order to infer the latent states, plan and make good decisions. Coping with partial observability in general is extremely challenging, as a number of worst-case statistical and computational barriers are known in learning Partially Observable Markov Decision Processes (POMDPs). Motivated by the problem structure in several physical applications, as well as a commonly used technique known as "frame stacking", this paper proposes to study a new subclass of POMDPs, whose latent states can be decoded by the most recent history of a short length $m$. We establish a set of upper and lower bounds on the sample complexity for learning near-optimal policies for this class of problems in both tabular and rich-observation settings (where the number of observations is enormous). In particular, in the rich-observation setting, we develop new algorithms using a novel "moment matching" approach with a sample complexity that scales exponentially with the short length $m$ rather than the problem horizon, and is independent of the number of observations. Our results show that a short-term memory suffices for reinforcement learning in these environments.

==> notations.tex <==
\RequirePackage{amsmath}

\ifx\proof\undefined 
\RequirePackage{amsthm}
\fi
\RequirePackage{bm} 
\RequirePackage{url}
\RequirePackage{color}


% bold alphabet 

\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
% \newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
% \newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sbb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

%%%%%%%%%%%%


%%%% calligraphic fonts

\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{{\mathcal{S}}}
\newcommand{\Tcal}{{\mathcal{T}}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%% Widely accepted definitions %%%%%%%%%%%%%%%

\newcommand{\CC}{\mathbb{C}} % Complex numbers
\newcommand{\EE}{\mathbb{E}} % Expectation
\newcommand{\VV}{\mathbb{V}} % Variance
\newcommand{\II}{\mathbb{I}} % Indicator
\newcommand{\KK}{\mathbb{K}} % Arbitrary field
\newcommand{\LL}{\mathbb{L}} % Loss
\newcommand{\MM}{\mathbb{M}} % Median
\newcommand{\NN}{\mathbb{N}} % Natural numbers
\newcommand{\OO}{\mathbb{O}} % Emission 
\newcommand{\PP}{\mathbb{P}} % Probability
\newcommand{\QQ}{\mathbb{Q}} % Rationals
\newcommand{\RR}{\mathbb{R}} % Real numbers
\newcommand{\ZZ}{\mathbb{Z}} % Integers
\newcommand{\XX}{\mathbb{X}} %
\newcommand{\YY}{\mathbb{Y}} %

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%% Some standard definitions

\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand*{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\DeclareMathOperator*{\Var}{{\rm Var}}
\DeclareMathOperator*{\Cor}{Corr}
\DeclareMathOperator*{\Cov}{Cov}
\DeclareMathOperator*{\indic}{\mathbbm{1}}  % Indicator
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}  
                                                        
\newcommand*{\zero}{{\bf 0}}
\newcommand*{\one}{{\bf 1}}

\newcommand*{\Risk}{{\rm Risk}}
\newcommand*{\Bias}{{\rm Bias}}

\newcommand{\pen}{{\rm pen}}
\newcommand{\diag}{{\rm diag}}

\def\iid{{\it i.i.d.}}
\newcommand{\iidsim}{\stackrel{{iid}}{\sim}}
\def\bks{\backslash}



%%%%%%%% bold greek letters %%%%%%%%%%

\newcommand*{\alphab}{\bm{\alpha}}
\newcommand*{\betab}{\bm{\beta}}
\newcommand*{\Sigmab}{\bm{\Sigma}}
\newcommand*{\Omegab}{\bm{\Omega}}
\newcommand*{\omegab}{\bm{\omega}}
\newcommand*{\Gammab}{\bm{\Gamma}}
\newcommand*{\Psib}{\bm{\Psi}}
\newcommand*{\Thetab}{\bm{\Theta}}
\newcommand*{\thetab}{\bm{\theta}}
\newcommand*{\taub}{\bm{\tau}}
\newcommand*{\epsilonb}{\bm{\epsilon}}
\newcommand*{\etab}{\bm{\eta}}
\newcommand*{\xib}{\bm{\xi}}
\newcommand*{\gammab}{\bm{\gamma}}
\newcommand*{\deltab}{\bm{\delta}}
\newcommand*{\Deltab}{\bm{\Delta}}
\newcommand*{\mub}{\bm{\mu}}
\newcommand*{\rhobb}{\bm{\rho}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%% Norms

\newcommand{\orlnorm}[2]{||#1||_{\Psi_{#2}}}
\newcommand{\norm}[1]{||#1||}
\newcommand{\bignorm}[1]{\bigg|\bigg|#1\bigg|\bigg|}
\newcommand{\opnorm}[2]{| \! | \! | #1 | \! | \! |_{{#2}}}

%%%%% Dot product
\newcommand{\dotp}[2]{\langle{#1},{#2}\rangle}

%%%%  brackets
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}

%%%%%%%%%  Other commands

\newcommand{\mcomment}[1]{\marginpar{\tiny{#1}}}
\newcommand{\fcomment}[1]{\footnote{\tiny{#1}}}


%%%%%%%%  amsmath %%%%%%%%%%


\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\QED\undefined
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\ifx\proof\undefined
\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
%\newenvironment{proof}{\emph{Proof. }}{ \hfill \QED}
\fi

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\fi
\ifx\assumption\undefined
\newtheorem{assumption}{Assumption}
\fi
\ifx\example\undefined
\newtheorem{example}{Example}
\fi
\ifx\property\undefined
\newtheorem{property}{Property}
\fi
\ifx\lemma\undefined
\newtheorem{lemma}[theorem]{Lemma}
\fi
\ifx\proposition\undefined
\newtheorem{proposition}[theorem]{Proposition}
\fi
\ifx\remark\undefined
\newtheorem{remark}[theorem]{Remark}
\fi
\ifx\corollary\undefined
\newtheorem{corollary}[theorem]{Corollary}
\fi
\ifx\definition\undefined
\newtheorem{definition}[theorem]{Definition}
\fi
\ifx\conjecture\undefined
\newtheorem{conjecture}[theorem]{Conjecture}
\fi
\ifx\fact\undefined
\newtheorem{fact}[theorem]{Fact}
\fi
\ifx\claim\undefined
\newtheorem{claim}[theorem]{Claim}
\fi
\ifx\claim\undefined
\newtheorem{observation}[theorem]{Observation}
\fi
\ifx\assum\undefined
\newtheorem{assum}[theorem]{Assumption}
\fi
\ifx\hypothesis\undefined
\newtheorem{hypothesis}[theorem]{Induction Hypothesis}
\fi


%%%% James's

\newcommand*{\cut}{\textrm{cut}}
\newcommand*{\out}{\textrm{out}}


%%%% Akshay's
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand{\order}{\ensuremath{O}}
\newcommand{\otil}{\ensuremath{\tilde{\order}}}
\newcommand{\defeq}{:=}
\newcommand{\grad}{\nabla}
\newcommand{\dmid}{\;||\;}
\newcommand{\KL}{\mathrm{KL}}



%%%% prettyref

\usepackage{prettyref}
\newcommand{\pref}[1]{\prettyref{#1}}
\newcommand{\pfref}[1]{Proof of \prettyref{#1}}
\newcommand{\savehyperref}[2]{\texorpdfstring{\hyperref[#1]{#2}}{#2}}
\newrefformat{hypothesis}{\savehyperref{#1}{Induction Hypothesis~\ref*{#1}}}
\newrefformat{eq}{\savehyperref{#1}{\textup{(\ref*{#1})}}}
\newrefformat{eqn}{\savehyperref{#1}{Equation~\ref*{#1}}}
\newrefformat{lem}{\savehyperref{#1}{Lemma~\ref*{#1}}}
\newrefformat{def}{\savehyperref{#1}{Definition~\ref*{#1}}}
\newrefformat{line}{\savehyperref{#1}{line~\ref*{#1}}}
\newrefformat{thm}{\savehyperref{#1}{Theorem~\ref*{#1}}}
\newrefformat{corr}{\savehyperref{#1}{Corollary~\ref*{#1}}}
\newrefformat{sec}{\savehyperref{#1}{Section~\ref*{#1}}}
\newrefformat{app}{\savehyperref{#1}{Appendix~\ref*{#1}}}
\newrefformat{assum}{\savehyperref{#1}{Assumption~\ref*{#1}}}
\newrefformat{ex}{\savehyperref{#1}{Example~\ref*{#1}}}
\newrefformat{fig}{\savehyperref{#1}{Figure~\ref*{#1}}}
\newrefformat{alg}{\savehyperref{#1}{Algorithm~\ref*{#1}}}
\newrefformat{rem}{\savehyperref{#1}{Remark~\ref*{#1}}}
\newrefformat{conj}{\savehyperref{#1}{Conjecture~\ref*{#1}}}
\newrefformat{prop}{\savehyperref{#1}{Proposition~\ref*{#1}}}
\newrefformat{proto}{\savehyperref{#1}{Protocol~\ref*{#1}}}
\newrefformat{prob}{\savehyperref{#1}{Problem~\ref*{#1}}}
\newrefformat{claim}{\savehyperref{#1}{Claim~\ref*{#1}}}
\newrefformat{observation}{\savehyperref{#1}{Observation~\ref*{#1}}}



%%% Yonathan - New notations%%%%

\newcommand{\rng}{{\mathrm{Rng}}}
\newcommand{\mmPi}[1]{{#1}^{\phi_\star}}

%%% Sobhan - GOLF Paper %%%

\newcommand{\regret}{{\mathrm{Regret}}}


\newcommand{\EcalII}{\mathcal{E}_{\textrm{V}}}


\newcommand{\reghat}{ {\widehat{\rm Reg}}}
\newcommand{\reg}{ {\mathrm{Reg}}}
\newcommand{\Rcalhat}{\hat{\mathcal{R}}}

\newcommand{\cU}{\mathcal{U}}
\newcommand{\uncert}{\mathcal{U}^*}
\newcommand{\normsigma}[2]{\norm{#1}_{\Sigma_{#2}}}
\newcommand{\normsigmainverse}[2]{\norm{#1}_{\Sigma_{#2}^{-1}}}
\newcommand{\phibar}{\bar{\phi}}


\newcommand{\strap}{s_{\rm trap}}


\newcommand{\T}{{\mathbb{T}}}
\newcommand{\Tstar}{{\mathbb{T}}^\star}

\newcommand{\Mhat}{\widehat{\mathcal{M}}}
\newcommand{\TM}{{{\mathbb{T}}^{\Mcal_h}}}
\newcommand{\TMC}{{{\mathbb{T}}^{\Mhat_h}}}

\newcommand{\OnOracle}{{\mathcal{O}}}
\newcommand{\fstar}{f^\star}
\newcommand{\pistar}{\pi^\star}
\newcommand{\unif}{\mathrm{Uniform}}

\newcommand{\olive}{\textsc{Olive}}
\newcommand{\golf}{\textsc{Golf}}
\newcommand{\golfII}{\textsc{Golf}-II}
%\newcommand{\algx}{{${\mathsf{LCGO}}$}}
\newcommand{\algx}{\golf}
\newcommand{\ourslong}{{Local-Confidence Global-Optimism}}
\newcommand{\eleanor}{\textsc{Eleanor}}

\newcommand{\eludim}{\dim_\mathrm{E}}
\newcommand{\dedim}{\dim_\mathrm{DE}}
\newcommand{\BEdim}{\dim_\mathrm{BE}}
\newcommand{\deber}{\textsf{DE}}
\newcommand{\be}{\textsf{BE}}
\newcommand{\deberdim}{$\dim_{\rm{BE}}$}
\newcommand{\bedim}{$\dim_{\rm{BE}}$}
\newcommand{\bedimII}{$\dim_{\rm{VBE}}$}
\newcommand{\bendim}{$\dim_{\rm{BEN}}$}


\newcommand{\dirac}{\Delta}
\newcommand{\Err}{\mathrm{Err}}

\newcommand{\Ffrak}{\mathfrak{F}}
\newcommand{\hatberrII}[1]{\hat{\Ecal}_{\textrm V}(#1)} 
\newcommand{\tildeberrII}[1]{\tilde{\Ecal}_{\textrm V}(#1)}


\newcommand{\nact}{n_\text{act}}
\newcommand{\nelim}{n_\text{elim}}
\newcommand{\zetaact}{\zeta_\text{act}}
\newcommand{\zetaelim}{\zeta_\text{elim}}
\newcommand{\empVf}[1]{\hat{V}_{#1}}
\newcommand{\berr}[1]{\Ecal(#1)}
\newcommand{\ft}[1]{f_{#1}}
\newcommand{\pit}[1]{\pi_{#1}}
\newcommand{\hatberr}[1]{\hat \Ecal(#1)} 

\newcommand{\dlin}{{d_{\text{lin}}}}
\newcommand{\dE}{d_{\text{E}}}
\newcommand{\bmu}{\boldsymbol{\mu}}
% \newcommand{\norm}[1]{\|{#1} \|}



==> sections/mmpolicy.tex <==
\todo[inline]{I believe we need to mention that these policies $\mu$, $\nu$ and $\tilde{\pi}$ only appear in analysis and the algorithm itself always uses $m$-step greedy polices  w.r.t some function $\Fcal$}

Towards developing a general purpose RL algorithms for $m$-step decodable POMDPs we uncover a low-rank structure of this model. To do so, we define the \emph{moment-matching policy} that, conditioning on the unobserved latent states and observations, induces similar action distribution . Building on this structural result we later develop algorithms that learns a near optimal policy for $m$-step decodable POMDPs in the function approximation setting.

\begin{definition}[Moment-Matching Policy] 
\label{def:moment_matching} Denote $m(h) = h-m+1$; Fix $h \in [H]$ and for $h' \in [m(h),h]$ we define  
$$
	x_{h'}=\big(s_{m(h):h'},o_{m(h):h'},a_{m(h):h'-1}\big) \in \Xcal_l,
$$
where $\Xcal_l = \Scal^l \times \Ocal^l \times \Acal^{l-1}$ and $l = h'-m(h)$. For a $m$-step policy $\pi$ and $h \in [H]$, we define the moment matching policy $\mu^{\pi,h}=\{\mu^{\pi,h}_{h'}: \Xcal_l \rightarrow \Delta (\Acal) \}_{h'=m(h)}^h$ as following:
\begin{equation*}
\begin{aligned}
	\mu^{\pi,h}_{h'}(a_{h'} \mid x_{h'})  
	\defeq \EE_\pi[ \pi_{h'}(a_{h'} \mid z_{h'}) \mid x_{h'}].
\end{aligned}
\end{equation*}	
By \cref{asm:nstep_decode}, states and therefore $x_h'$ is decodable by the history of actions and observations, therefore we can have
\begin{equation*}
	\begin{aligned}
		\nu^{\pi,h}_{h'}(a_{h'} \mid o_{1:h'}, a_{1:h'-1}) 
		\defeq \mu^{\pi,h}_{h'} (a_{h'} \mid x_h').
	\end{aligned}
\end{equation*}
%where $\tilde{x}_{h'}$ is defined based on the true decoder; namely,
%\begin{equation*}
%	\begin{aligned}
%		&\tilde{x}_{h'}=\big(\tilde{s}_{h-m+1:h'},o_{h-m+1:h'},a_{h-m+1:h'-1}\big) \in \Xcal_j,\\
%		&\tilde{s}_{h'}=\phi^*(z_{h'}).
%	\end{aligned}
%\end{equation*}
\end{definition}



  
With the above definition at hand, we establish two key properties.
\begin{lemma}
	\label{lem:main_momentmatching}
	For a fixed $h \in [H]$ and fixed $m$-step policies $\pi,\bar{\pi}$, define policy $\tilde{\pi}^h$ which takes first $m(h)-1$ actions from $\pi$ and remaining actions from $\nu^{\bar{\pi},h}$, i.e. $\tilde{\pi}^h= \pi \circ_{m(h)} \nu^{\pi,h}$. Then we have, 
	\begin{enumerate}
		\item For any $z_h \in \Zcal_h$, $P_{\pi}(z_h)=P_{\tilde{\pi}^h}(z_h)$
		\item For any function $g: \Zcal_h \rightarrow [0,1]$,
		\begin{equation*}
			\EE_{\tilde{\pi}^h}[g(z_h)]= \langle \zeta_h(\pi) , \xi_h(g,\bar{\pi})\rangle,
		\end{equation*}
		where $\zeta_h(\pi),\xi_h(g,\bar{\pi}) \in \mathbb{R}^S$ satisfying $\norm{\zeta_h(\pi)} \leq 1$ and $\norm{\xi_h(g,\bar{\pi})} \leq \sqrt{S}$.
	\end{enumerate}
\end{lemma}

 Lemma establishes two key properties: First, policies $\pi$ and $\tilde{\pi}$ induce same distribution over $z_h$. Second, expectation of any function $g: \Zcal_h \times \Acal \rightarrow [0,1]$ under policy $\tilde{\pi}$ has low-rank structure and can be factorized with rank $S$.


\todo[inline]{I believe we need to mention that these policies $\mu$, $\nu$ and $\tilde{\pi}$ only appear in analysis and the algorithm itself always uses $m$-step greedy polices  w.r.t some function $\Fcal$}


\todo[inline]{In our algorithm we choose $g = (f_h-\Tcal f_{h+1})(z_h, \pi_f(z_h))$}
\todo[inline]{isn't $\xi_h(g)$ depends on $\nu$ and the policy at the $h^{th}$ time step too?}


\todo[inline]{TODO: show that the 1-step decoupling does not have low-rank structure / negative result for the Billinear class.}



%
%Given any policy $\pi$ the induced moment-matching policy $\mmPi{\pi}$ is defined as follows. 
%\begin{definition}[Moment-Matching Policy]
%Fix a policy $\pi: \Zcal_h\times[H]\rightarrow \Delta(\Acal)$. The moment-matching policy with respect to $\pi$, denoted by $\mmPi{\pi}$, is a mapping  $\Scal\rightarrow \Delta(\Acal)$. Furthermore, it satisfies that for all $z\in \Zcal$ such that $\PP_{\pi_f}\rbr{z_h=z}>0$ and for all $a\in \Acal$, it holds that
%\begin{align*}
%\mmPi{\pi}(a|s) = \PP_{\pi}\rbr{a_h=a | \phi^\star(z) = s}.
%\end{align*}
%\end{definition} 
%In words, the moment matching policy $\pi^{\phi^\star}$ induced by $\pi$ has the same action distribution conditioning on any unobservable latent state $s\in \Scal$.
%

%With the above definition at hand, we uncover the following low-rank structure of an $m$-step decodable POMDP.
%\begin{lemma}[Low-rank structure of $n$-step decodable POMDP]\label{lem: low rank decoupling}
%
%Let $g: \Zcal\times\Acal\rightarrow \mathbb{R}$ be any mapping from last $n$ observations and current action to a real number. Then, for any policy $\psi\circ_{h-n}\pi$ it holds that
%\begin{align*}
%\EE_{\psi\circ_{h-n}\pi} \sbr{g(z_h,a_h,z_{h+1})} = \inner{\nu(\psi)}{\xi(\mmPi{\pi},g)},
%\end{align*}
%where $\nu(\psi),\xi(\mmPi{\pi},g)\in \mathbb{R}^{S}$ such that $\nu(\psi)(s) = \PP_{\pi,h-n}\rbr{s}$ and $\xi(\mmPi{\pi},g)(s)= \EE_{\pi^{\phi^\star}}\sbr{ g(z_h,a_h)\mid s_{h-n} = s}$.
%\end{lemma}




==> sections/olive.tex <==

\begin{algorithm*}[h]
\caption{\olive\ for $n$-BMDP} \label{alg:algxII}
 \begin{algorithmic}[1]
% \STATE \textbf{Input}: Function Class $\Fcal$, Confidence parameter $\delta$
 \STATE \textbf{Initialize}:  $\Dcal_1,\dots,\Dcal_H\leftarrow \emptyset$, $\Bcal^0 \leftarrow \Fcal$.
 \STATE \textbf{Define}
$
    \Pi_\Phi := \{ \pi_\phi(\cdot \mid \phi(z)) : \pi_\phi: \Scal \mapsto \Delta(\Acal), \phi \in \Phi \} 
$
\FOR{\textbf{epoch} $k$ from $1$ to $K$} 
 \STATE \textbf{Choose policy} $\pi^k = \pi_{f^k}$, where $f^k = \argmax_{f \in \Bcal^{k-1}}f(x_1,\pit{f}(x_1))
 $.
 \STATE \textbf{Estimate} for all $h\in [H]$ $$\widehat{\Ecal}\rbr{\pi_k,f^k,h} = \frac{1}{N_{\mathrm{eval}}}\sum_{i=1}^{N_{\mathrm{eval}}} f^k_h(z_{h},\pi_k(z_{h})) - r_h - f^k_{h+1}\rbr{ z_{h+1},\pi_k(z_{h+1})}.$$
\STATE {\bf if} $\sum_{h}\widehat{\Ecal}\rbr{\pi_f,f,h} \leq \epsilon$ {\bf then} terminate and output $\pi_f$.
\FOR{\textbf{step} $h$ from $1$ to $H$}
\STATE \textbf{Collect}  $z_h=(x_{h-n+1},a_{h-n+1},\dots,x_h,a_h)$, $r_h$, and $x_{h+1}$ by executing $\pi^k$ at step $1,\ldots,h-n$ and taking  action uniformly at random at step $h-n+1,\dots,h$. 
\STATE \textbf{Augment} $\Dcal_h=\Dcal_h\cup (z_h,r_h,x_{h+1})$ for all $h\in[H]$.
\STATE \textbf{Estimate}  for all $\pi_\phi \in \Pi_\Phi$ and $f\in \Fcal$
\begin{align}
\widehat{\Ecal}_h(\pi_k, \pi_\phi,f) = \frac{1}{N} \sum_{i=1}^N \rbr{\prod_{j=1}^{n} \frac{\pi_\phi(a_{h-j} \mid z_{h-j})}{1/A}} (f(z_h, \pi_f(z_h)) - r_h - f(z_{h+1}, \pi_f(z_{h+1})).
\end{align}

\ENDFOR

\STATE \textbf{Update}
$
	\Bcal^{k}= \left\{ f \in \Bcal^{k-1}: \forall h\in [H],\pi_\phi\in \Pi_\Phi\  \abr{\widehat{\Ecal}_h\rbr{\pi_f,\pi_\phi,f,h}} \leq \epsilon \right\}.
$
\ENDFOR
\STATE \textbf{Output} $\pi^{\rm out}$ sampled uniformly at random from $\{\pi^k\}_{k=1}^{K}$.
 \end{algorithmic}
\end{algorithm*}


==> sections/proof_overview_backup.tex <==
%!TEX root = ../main.tex

In this section we elaborate on the challenges and provide a proof overview for~\pref{thm:golf_regret}.  We start by describing the difficulties in learning a near optimal policy for an $m$-step decodable POMDP. Specifically, we show that the Bellman rank can depend on the size of the observation space, and also that \olive~\cite{jiang2017contextual} requires $\Omega(O)$ samples to find an $o(1)$ optimal policy. 

Next, we expand on the proof technique. Central to our analysis is a structural result  of the $m$-step decodable POMDP model. We introduce the \emph{moment-matching policy} for a policy $\pi$, and show this construction implies an $m$-step decodable POMDP has a low rank structure. Relying on this observation, we generalize the analysis of \golf\ to the $m$-step decodable POMDP model.

\subsection{Challenges: Bellman Rank is Large}\label{sec: challenges}
The Bellman rank was introduced in~\cite{jiang2017contextual} as a complexity measure that characterizes tractability of RL with function approximations. Hence, the Bellman rank depends on both the underlying model $\Mcal$, with which the agent interacts, and the function class it is being given $\Fcal$. The authors also designed \olive~\cite{jiang2017contextual} and proved its sample complexity is bounded by the Bellman rank. It is known that many MDPs in which exploration is tractable, such as tabular MDPs, linear MDPs and block MDPs, have bounded Bellman rank.  

The next result proves that the Bellman rank of an $m$-step decodable POMDP with $m=2$ is lower bounded by the cardinality of the observation space $\Omega(O)$. Furthermore, it also shows that \olive\ needs at least $\Omega(O)$ samples to find an $O(1)$ optimal policy. This highlights the challenge in designing RL algorithm for the $m$-step decodable POMDP. Although \olive\ solves a $1$-step decodable POMDP -- namely, a block MDP -- it fails in solving an $m$-step decodable POMDP. 

\begin{proposition}[Bellman rank of $m$-step Decodable POMDP is Large]\label{prop: bellman rank of an m step dec pomdp is large}
There exists a $2$-step decodable POMDP $\Mcal$ and a function class $\Fcal$ such that the Bellman rank of $\rbr{\Mcal,\Fcal}$ is $\Omega(O)$. Additionally, \olive\ instantiated with $\Fcal$ requires $\Omega(O)$ samples to find an $o(1)$ optimal policy for~$\Mcal$.
\end{proposition}

Although the general purpose \olive\ algorithm fails in finding a near optimal policy of an $m$-step decodable POMDP,~\pref{thm:golf_regret} proves that $m$-\golf\ is able to so. 



\subsection{Proof Overview \& Moment Matching Policy}
\label{sec:moment_matching}

\begin{figure}
\label{fig: moment matching policy}
\includegraphics[width=0.45\textwidth]{./sections/mm_policy_crop.pdf}
\caption{An illustration of the dependency structure of a moment matching policy, depicted in red, and a regular policy, depicted in blue, in a $2$-step decodable POMDP. The moment matching policy $\mu^{\pi,h+1}$ selects action $a_h$ based on the state $s_h$ and observation $o_h$ to match the distribution $\PP^\pi[a_h \mid s_h,o_h]$. It breaks the dependence on the history by marginalizing out $(o_{h-1},a_{h-1})$, but correctly matches the distribution $\PP^\pi[o_{h+1},a_h,o_h]$. }
\end{figure}


We now describe our key novelty in establishing~\pref{thm:golf_regret}, which also shed light on the design of $m$-\golf. We identify an $S$-dimensional low rank structure in an $m$-step decodable POMDP. Relying on this structure we are able to generalize \golf 's analysis to prove~\pref{thm:golf_regret}.

Consider the Bellman error at the $h^{th}$ time step of a function $f\in \Fcal$ when executing roll-in policy $\pi$, given by
\begin{equation*}
	\Ecal_h(\pi,f) = \EE[(f_h-\Tcal_h f_{h+1})(z_h,\pi_f(z_h)) \mid a_{1:h-1} \sim \pi ].
\end{equation*}
Assuming the Bellman rank is $M$, implies that $\Ecal_h(\pi,f) = \inner{\zeta(\pi)}{\xi(f)}$ for some $\zeta,\xi\in \mathbb{R}^M$. This further allows to obtain a sample complexity gurantee of \olive\ that scales with $O(poly(M))$. However, as shown in~\pref{sec: challenges}, the Bellman rank of an $m$-step decodable POMDP may depend linearly in $O$, which may be arbitrarily larger than $S$. 

To establish the sample complexity of $m$-\golf\ we identify a surrogate Bellman error $\Ecal^\star_h(\pi,f)$ that has two key properties (see formal statement in~\pref{lem:golf_property}):
\begin{enumerate}
\item \emph{Coincides with standard bellman error when $\pi = \pi_f$}: $$\Ecal^\star_h(\pi_f,f) =  \Ecal_h(\pi_f,f).$$
\item  \emph{Embedded in $\mathbb{R}^S$}: $\Ecal^\star_h(\pi,f)$ can be embedded in an $S$-dimensional space. For some $\zeta(\cdot),\xi(\cdot)\in \mathbb{R}^S$, $$\Ecal^\star_h(\pi,f)= \inner{\zeta(\pi)}{\xi(f)}.$$ 
\end{enumerate}
Such result allows us to convert the Bellman error -- that upper bounds the optimality gap in optimistic algorithm -- to a surrogate Bellman error that can be embedded in a low-dimension space.  Building on this observation and generalizing analysis techniques of $m$-\golf\ allows us to prove~\pref{thm:golf_regret}.

We now describe the surrogate Bellman error $\Ecal^\star_h(\pi,f)$ in more details. 
We built $\Ecal^\star_h(\pi,f)$ by constructing an alternative sampling policy to $\pi$, $\pi\circ_{ m(h) } \nu^{\pi_f,h}$, and we define
\begin{align*}
&\Ecal^\star_h(\pi,f) \equiv \\
& \EE[(f_h-\Tcal_h f_{h+1})(z_h,\pi_f(z_h)) \mid a_{1:h-1} \sim \pi \circ_{ m(h) } \nu^{\pi_f,h} ].
\end{align*}
For a policy $\pi$, we construct $\nu^{\pi,h}_{h'}$ for $h'\geq h-m$ such that it matches the distribution of the action $a_{h'}$ conditioning on latent states and observations from time step $h-m+1$ to time step $h$ under the sampling process of $\pi$.  For this reason we refer to $\nu^{\pi}$ as the \emph{moment matching policy} for $\pi$ (see~\pref{fig: moment matching policy} for illustration). Formally, we define it as follows.

\begin{definition}[Moment-Matching Policy for $\pi$] 
\label{def:moment_matching} Denote $m(h) = h-m+1$; Fix $h \in [H]$ and for $h' \in [m(h),h]$ we define  
$$
	x_{h'}=\big(s_{m(h):h'},o_{m(h):h'},a_{m(h):h'-1}\big) \in \Xcal_l,
$$
where $\Xcal_l = \Scal^l \times \Ocal^l \times \Acal^{l-1}$ and $l = h'-m(h)$. For a $m$-step policy $\pi$ and $h \in [H]$, we define the moment matching policy $\mu^{\pi,h}=\{\mu^{\pi,h}_{h'}: \Xcal_l \rightarrow \Delta (\Acal) \}_{h'=m(h)}^h$ as following:
\begin{equation*}
\begin{aligned}
	\mu^{\pi,h}_{h'}(a_{h'} \mid x_{h'})  
	\defeq \EE_\pi[ \pi_{h'}(a_{h'} \mid z_{h'}) \mid x_{h'}].
\end{aligned}
\end{equation*}	
By \cref{asm:nstep_decode}, states and therefore $x_h'$ is decodable by the history of actions and observations, therefore we let
\begin{equation*}
	\begin{aligned}
		\nu^{\pi,h}_{h'}(a_{h'} \mid o_{1:h'}, a_{1:h'-1}) 
		\defeq \mu^{\pi,h}_{h'} (a_{h'} \mid x_h').
	\end{aligned}
\end{equation*}
\end{definition}

Recall that $\pi$ is an $m$-step policy that maps the recent $m$ observation-action sequence to an action. This implies that the observation at the $h^{th}$ time step may depend on observations prior to the $h-m^{th}$ time step; for example, since for $h-m \leq h'< h$ the action $a_{h'}$ is a function of observations before time $h-m^{th}$ time step. \sobcomment{I am not sure if this paragraph is necessary}

The moment matching policy allows us to break these dependencies while matching the distribution of $z_h$. For policy $\pi$ and $\bar{\pi}$, let $\tilde{\pi}^h =\pi\circ_{ m(h) }\nu^{\bar{\pi},h}$, we have:
\begin{enumerate}
\item \emph{Matches distribution:} If $\pi = \bar{\pi}$ $$\PP_{\tilde{\pi}^h}(z_h) = \PP_{\pi}(z_h).$$
\item \emph{Breaks dependencies:} For any $g:\Zcal_h \rightarrow [0,1]$ $$\EE_{\tilde{\pi}^h}(g(z_h) ) = \sum_{s_{m(h)}}\PP_{\pi}(s_{m(h)}) \EE_{\mu^{\bar{\pi},h}}(g(z_h) \mid s_{m(h)}).$$
\end{enumerate}  
With these properties,  it readily follows that $(1)$ $\Ecal_h(\pi_f,f) = \Ecal^\star_h(\pi_f,f) $, and that $(2)$ $\Ecal^\star_h(\pi,f)$ can be embedded in $\mathbb{R}^S$; thus, the two key properties that $\Ecal^\star_h(\pi,f)$ is supposed to satisfy, hold.


The aforementioned observations implies that instead of measuring the Bellman error of $f$ with respect to $\pi_f$ we can, alternatively, measure it with respect to $\pi \circ_{ m(h) }\nu^{\pi_f,h}$ which is a low-rank object. Unfortunately, we do not have access to $\nu^{\pi_f,h}$ without prior knowledge on the true decoder $\phi^\star$. Nevertheless, $m$-\golf\ bypasses this problem by executing a uniform action for $m$ time steps, instead of executing $\nu^{\pi_f,h}$; taking the uniform action for the last $m$ time steps allows us to upper bound $\Ecal^\star_h(\pi,f)$ using the importance sampling trick, while only suffering an $A^m$ degradation in the sample complexity. Such factor is necessary according to~\pref{prop: tabular_lower}.  


